Inferring Sparsity: Compressed Sensing using Generalized Restricted Boltzmann Machines

In this work, we consider compressed sensing reconstruction from $M$ measurements of $K$-sparse structured signals which do not possess a writable correlation model. Assuming that a generative statistical model, such as a Boltzmann machine, can be trained in an unsupervised manner on example signals, we demonstrate how this signal model can be used within a Bayesian framework of signal reconstruction. By deriving a message-passing inference for general distribution restricted Boltzmann machines, we are able to integrate these inferred signal models into approximate message passing for compressed sensing reconstruction. Finally, we show for the MNIST dataset that this approach can be very effective, even for $M < K$.

==> Makefile <==
FILENAME = grbm-amp
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf
LOG_FILE = $(FILENAME).log

PAPERSIZE = a4
# PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	pdflatex -jobname $(FILENAME) main
	find . -regex ".*aux" | while read auxfile; \
	do \
		if grep citation $$auxfile; then \
		echo $$auxfile >> bibbuild.log; \
		echo "------------------------" >> bibbuild.log; \
		bibtex $$auxfile >> bibbuild.log; \
		echo " " >> bibbuild.log;\
		fi; \
	done
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log	
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log

arxiv: main
	rm *.toc
	rm *.pdf
	rm *.log
	rm *.blg
	rm *.aux


dvi2pdf:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.4 \
		$(PS_FILE) $(PDF_FILE)

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

print: main
	dvips main

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

compress: clean
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Compressing files in $$i" ; \
	for j in $(COMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(COMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

uncompress:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo Uncompressing files in $$i ; \
	for j in $(UNCOMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(UNCOMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

